A Population of Radio-loud Narrow Line Seyfert 1 Galaxies with Blazar-like Properties?

(abridged) We present a comprehensive study of a sample of 23 genuine radio-loud NLS1 galaxies which have the radio-loudness parameters greater than 100. The radio sources of the sample are ubiquitously compact. A significant fraction of these objects show interesting radio to X-ray properties that are unusual to most of the previously known radio-loud NLS1 AGN, but are reminiscent of blazars. These include flat radio spectra, large amplitude flux and spectral variability, compact VLBI cores, very high brightness temperatures derived from variability, enhanced optical emission in excess of the normal ionising continuum, flat X-ray spectra, and blazar-like SEDs. We interpret them as evidence for the postulated blazar nature of these very radio-loud NLS1 AGN, which might possess at least moderately relativistic jets. Intrinsically, some of the objects have relatively low radio power and would have been classified as radio-intermediate AGN. The black hole masses are estimated to be within 10^{6-8}Msun, and the inferred Eddington ratios are around unity. The results imply that radio-loud AGN may be powered by black holes with moderate masses (10^{6-7}Msun) accreting at high rates. We find that a significant fraction of the objects, despite having strong emission lines, resemble high-energy peaked BL Lacs (HBL) in their SED. Given the peculiarities of blazar-like NLS1 galaxies, questions arise as to whether they are plain downsizing extensions of normal radio-loud AGN, or whether they form a previously unrecognised population.

==> astroph_abs.tex <==
We present a comprehensive study of a sample of 23 genuine radio-loud NLS1
galaxies which have the radio-loudness parameters greater than 100. The radio
sources of the sample are ubiquitously compact. A significant fraction of these
objects show interesting radio to X-ray properties that are unusual to most of
the previously known radio-loud NLS1 AGN, but are reminiscent of blazars. These
include flat radio spectra, large amplitude flux and spectral variability,
compact VLBI cores, very high brightness temperatures derived from variability,
enhanced optical emission in excess of the normal ionising continuum, flat X-ray
spectra, and blazar-like SEDs. We interpret them as evidence for the postulated
blazar nature of these very radio-loud NLS1 AGN, which might possess at least
moderately relativistic jets. Intrinsically, some of the objects have relatively
low radio power and would have been classified as radio-intermediate AGN. The
black hole masses are estimated to be within 10^{6-8}Msun, and the inferred
Eddington ratios are around unity. The results imply that radio-loud AGN may be
powered by black holes with moderate masses (10^{6-7}Msun) accreting at high
rates. We find that a significant fraction of the objects, despite having strong
emission lines, resemble high-energy peaked BL Lacs (HBL) in their SED. Given
the peculiarities of blazar-like NLS1 galaxies, questions arise as to whether
they are plain downsizing extensions of normal radio-loud AGN, or whether they
form a previously unrecognised population.

